Model Selection for Treatment Choice: Penalized Welfare Maximization

This paper studies a penalized statistical decision rule for the treatment assignment problem. Consider the setting of a utilitarian policy maker who must use sample data to allocate a binary treatment to members of a population, based on their observable characteristics. We model this problem as a statistical decision problem where the policy maker must choose a subset of the covariate space to assign to treatment, out of a class of potential subsets. We focus on settings in which the policy maker may want to select amongst a collection of constrained subset classes: examples include choosing the number of covariates over which to perform best-subset selection, and model selection when approximating a complicated class via a sieve. We adapt and extend results from statistical learning to develop the Penalized Welfare Maximization (PWM) rule. We establish an oracle inequality for the regret of the PWM rule which shows that it is able to perform model selection over the collection of available classes. We then use this oracle inequality to derive relevant bounds on maximum regret for PWM. An important consequence of our results is that we are able to formalize model-selection using a "hold-out" procedure, where the policy maker would first estimate various policies using half of the data, and then select the policy which performs the best when evaluated on the other half of the data.

==> conclusion.tex <==
In this paper, we introduced a new statistical decision rule for the treatment assignment problem, which we call the Penalized Welfare Maximization (PWM) rule. Our rule builds on the Empirical Welfare Maximization Rule of \cite{kt2015}, which is designed for situations where treatment allocation is exogenously constrained. The PWM rule is designed for settings where the policy maker may want to choose amongst a collection of such constrained classes. We established an oracle inequality for the regret of the PWM rule which shows that it is able to perform model selection over the collection of available classes. We then applied this result to two examples: the choice of the number of covariates when performing best-subset selection, and the selection of an approximating class in a sieve.

Moving forward, we have identified some areas that we feel are worth further study. In general, implementing PWM is computationally challenging; from a practical perspective, practitioners may find it convenient to have a software package that can implement PWM in a few important examples. In particlar, decision/regression trees are becoming popular for the estimation of treatment effects, and as we illustrate in Appendix \ref{sec:appendixB} could serve as a useful approximating classes in our setting. We hope to further study the use of decision trees in the treatment assignment problem, as well as implement a software package that implements decision-tree based rules for practitioners.
